Interactive Learning from Activity Description

We present a novel interactive learning protocol that enables training request-fulfilling agents by verbally describing their activities. Unlike imitation learning (IL), our protocol allows the teaching agent to provide feedback in a language that is most appropriate for them. Compared with reward in reinforcement learning (RL), the description feedback is richer and allows for improved sample complexity. We develop a probabilistic framework and an algorithm that practically implements our protocol. Empirical results in two challenging request-fulfilling problems demonstrate the strengths of our approach: compared with RL baselines, it is more sample-efficient; compared with IL baselines, it achieves competitive success rates without requiring the teaching agent to be able to demonstrate the desired behavior using the learning agent's actions. Apart from empirical evaluation, we also provide theoretical guarantees for our algorithm under certain assumptions about the teacher and the environment.

==> sections/regret_analysis.tex <==
\section{Theoretical Analysis}

We analyze the regret guarantees for $\mainalg$.

\patrick{looks like notation has not caught up with earlier sections? specifically mu vs P*?}
For a given reward function $R \in \Rcal$, we define $q(e \mid R)$ as the uniform probability over all episodes that achieve optimal return under $R$. We use $q$ to lift our model $\mu$ from reward to over episodes. Formally, for a given episode $e \in \Ecal$, description $d \in \Vcal^\star$, and start state $s_0$, we define: 

\khanh{this comment is making the algorithm lines red. they will go back to black when we remove the comment. don't worry}
\begin{equation*}
    \mu(e, d, s_0) = \sum_{R \in \Rcal} q(e \mid R) \mu(R, d, s_0).
\end{equation*}
We also define $\mu(e)$ as the marginal distribution over episodes and $\mu(d \mid e)$ as the conditional distribution over $d$ given $e$. We define $\mu(d \mid e)$ as the \emph{problem description model}.

However, a critical step is missing in connecting the role of the teacher model to the problem model. Our goal is to rule out situations where the teacher model is completely different from the problem model. We, therefore, require these two models to be similar, such that following the teacher model enables solving the problem. We accomplish this with the following definition:

\begin{definition}[$\alpha$-consistent teacher] We define $\PP_T$ to be $\alpha$-consistent if for all $e \in \Ecal$, we have:
\begin{equation*}
    \TV{\mu(d \mid e) - \PP_T(d \mid e)} \le \alpha
\end{equation*}
\end{definition}

\dipendra{Possibly not true if teacher is pragmatic and world is not. E.g., hypothesis are ``birds, bats" and descriptors are ``eggs, flies". Say the task was to pick "birds", world says "flies" and the agent picks the "bat", and the teacher would say "flies", and if the agent picks the "bird" and then the teacher would say "eggs".}
\dipendra{if literal teacher is close to the world then pragmatic teacher is close to the pragmatic version of world.}

We define regret $\Reg$ of the algorithm after $N$ rounds as:
\begin{equation*}
    \Reg(N) \defeq \sum_{n=1}^N \left(V^\star(d_n, s_{0, n}) - \hat{V}(\pi_n, d_n, s_{0, n}, R_n)\right).
\end{equation*}

\begin{theorem}[Main Result] Fix $\delta \in (0, 1)$. Then with probability at least $1-\delta$, the regret of $\mainalg$ is given by:
\begin{equation*}
    \Reg(N) \le ????
\end{equation*}
\end{theorem}

We defer the proof and complete analysis to~\pref{app:regret-analysis}.
